Robust Markov decision processes under parametric transition distributions

This paper considers robust Markov decision processes under parametric transition distributions. We assume that the true transition distribution is uniquely specified by some parametric distribution, and explicitly enforce that the worst-case distribution from the model is uniquely specified by a distribution in the same parametric family. After formulating the parametric robust model, we focus on developing algorithms for carrying out the robust Bellman updates required to complete robust value iteration. We first formulate the update as a linear program by discretising the ambiguity set. Since this model scales poorly with problem size and requires large amounts of pre-computation, we develop two additional algorithms for solving the robust Bellman update. Firstly, we present a cutting surface algorithm for solving this linear program in a shorter time. This algorithm requires the same pre-computation, but only ever solves the linear program over small subsets of the ambiguity set. Secondly, we present a novel projection-based bisection search algorithm that completely eliminates the need for discretisation and does not require any pre-computation. We test our algorithms extensively on a dynamic multi-period newsvendor problem under binomial and Poisson demands. In addition, we compare our methods with the non-parametric phi-divergence based methods from the literature. We show that our projection-based algorithm completes robust value iteration significantly faster than our other two parametric algorithms, and also faster than its non-parametric equivalent.

==> X2_LR_notes.tex <==
\newpage
\section{Literature Review Notes}

Some references with notes to follow. Firstly, initial papers:
\begin{enumerate}
    \item \cite{Satia73}: first (I think) formulation of RMDPs. Ambiguity sets allocated an upper and lower bound to each probability. Game theoretic and Bayesian formulations. Algorithm presented is a two-step algorithm consisting of policy evaluation followed by policy improvement. Algorithm proved $\epsilon$-optimal, converges in finite number of iterations. Separate algorithm formed for Bayesian formulation. No value iteration, strange format for ambiguity set.
    \item \cite{GIVAN2000}: bounded parameter MDPs, i.e.\ a collection of exact MDPs resulting from bounding transition probabilities and rewards. Define new concept of interval value functions which is essentially an interval defined by the minimum and maximum value of the value functions of all MDPs defined by the interval bounds. Optimistic and pessimistic policies optimise upper and lower bounds respectively. Interval policy evaluation algorithm presented. Interval value iteration also presented: it updates both upper and lower bounds of value function in each iteration. Not a convenient or readable framework. 
    \item \cite{bagnell2001solving}: RMDPs similar to how we see them now. Convex, compact ambiguity sets. This contains interval ambiguity sets. Robust value iteration firstly finds the worst-case distribution for the current value function for each state and action (because deterministic policies) and then updates the values in the next step. Convergence proof provided.
    \item \cite{Nilim05}: First finite horizon robust DP. Rectangular ambiguity sets. I believe this is the introduction of robust DP. Another repeated game type formulation, with actions selected assuming that the worst-case distribution will be selected, then the adversary selecting the worst-case distribution for the action. Robust DP algorithm separates these two actions, finding worst-case value by bisection. Formal theorem for robust Bellman recursion (RVI) proposed, with theoretical results showing convergence and that there is an optimal stationary deterministic policy, and that the worst-case distribution is always selected by minimising the reward for the action chosen. Optimality result given for robust value iteration with the tolerance given by $(1-\nu)\epsilon/2\epsilon$. Ambiguity sets: likelihood models i.e.\ distributions under which the observed data have a high likelihood, maximum a posteriori models i.e.\ adjusting likelihood by some prior information, KLD ambiguity sets (entropy) presented as main AS's. Dual reformulations for value functions presented along with bisection algorithms for these problems. Only dualises the inner problem, i.e.\ distribution separation problem. Other AS's discussed include interval bound sets, ellipsoidal models.
    \item \cite{Iyengar05}: Rectangular ambiguity sets assumed. Proof of robust Bellman equations provided (don't think they had been seen before). Then infinite horizon is also covered. Robust value iteration described. Theoretical results established throughout the paper. Policy evaluation and iteraton also studied. Most formal presentation, with computational complexity also studied. First time distance based ambiguity sets are presented, with this paper looking at KLD sets and then a modified $\chi^2$ set is derived from using the distance as an upper bound on the KLD measure. They use these sets to reformulate the distribution separation problem via Lagrange duality to remove the ambiguity set constraint. Also studied $L_1$ norm ambiguity sets. Show equivalence of the RMDP with two-person zero sum games with perfect information.
    \item \cite{Mannor07}: study of the bias and variance in value function estimates resulting from using the esimated distributions instead of the true distributions. Even for a large number of samples, the value functions have large standard deviations. 
    \item \cite{Delage10}: argue that the RMDP approach generates conservative solutions. They instead use a Bayesian framework. Parameters considered as random variables. Does not actually use ambiguity sets, does not assume they lie in any set. It actually seems as though they treat the uncertain parameters as random variables from parametric distributions with known prior parameters. The parameter estimates are updated in a Bayesian fashion. Slightly similar to PDRO, but a worst-case approach is not taken. Model used here is a chance-constrained model. This is because they choose to optimise some upper percentile of the expected reward. Problem has an SCP reformulation for Gaussian parameters.
    \item \cite{Wiesemann13}: often-cited RMDP paper. Uses statistical estimation based on observation histories (not transition sampling) in order to construct confidence regions for use as ambiguity sets. They say these are much easier to obtain in practice. They also do not use any approximations of the RMDP, which apparently prior works did use. Rectangular ambiguity sets where probabilities are affine functions of some parameter $\xi$, of the form $\bm{P}_{s, a} = p^{\xi}(\cdot|s, a) = \bm{k}_{s, a} + \bm{K}_{s, a}\xi$. Complexity results derived for $s$-rectangular ambiguity sets, it seems as though their methods are less complex because their formulations can be solved using only second-order cone programs. Useful citation: by \cite{Wiesemann13}, solving the RMDP under $s$-rectangular ambiguity sets is equivalent to computing the fixed point of the Bellman operator, thus allowing a value iteration (VI) algorithm. (quoted from~\cite{Grand_Clement_Kroer_2021}).
\end{enumerate}
Development of ambiguity sets:
\begin{enumerate}
    \item \cite{le2007robust}: seemingly the first use of $s$-rectangular ambiguity sets.
    \item \cite{derman2021twice}: find equivalence relationships between twice-regularised MDPs and robust MDPs. A regularised MDP is an MDP whose Bellman evaluation operator is modified by some convex function. The authors show that strong duality exists between twice-regularised and robust MDPs, meaning that the optimal value of a RMDP can be solved via solving a twice-regularised MDP. The benefit of this is that twice-regularised MDPs are much faster to solve. The framework covers reward-robust MDPs (which are equivalent to once-regularised MDPs) and general robust MDPs. Ambiguity sets: $s$-rectangular ambiguity sets with ($\ell_2$) norm-based distance measure. Not distance from a nominal, just norm of a distribution.
    \item \cite{goyal2022robust}: non-rectangular ambiguity sets. They presented factor-matrix ambiguity sets - the distributions in this set are convex combinations of some common underlying factors with fixed coefficients. Each factor $\bm{w}_i$ for $i \in [r]$ is a distribution itself over the next state, and the distribution is given by $\bm{P}_{s, a} = \sum_{i=1}^r u^i_{s, a} \bm{w}^i$. The vector $\bm{W} = (\bm{w}_1,\dots,\bm{w}_r)$ is a member of some underlying set $\m{W}$. It is assumed that $\m{W}$ is $r$-rectangular, but this does not mean the resulting ambiguity set is $s$-rectangular or $(s,a)$-rectangular. They show that any ambiguity set can be reformulated as a factor matrix ambiguity set (probably not parametric ones though). They show strong minmax duality for their problem and use this to develop a fast algorithm.
    \item \cite{NEURIPS2018_7ec0dbee} use ambiguity sets constructed by bounding the marginal moments of state-action feature functions over entire MDP trajectories. They take samples of the feature functions and only consider parameters that have the same expectation as the one observed. They then develop algorithms for the RMDP that consist of solving a collection of MDPs. 
\end{enumerate}
Algorithms for $s$-rectangular ambiguity sets:
\begin{enumerate}
    \item \cite{Ho21}: $s$-rectangular ambiguity sets defined by the $L_{\infty}$ norm, i.e. $\|\bm{x}\|_{\infty} =  \max_{n} |x_n|$. Initial focus of the paper is on efficiently solving the distribution separation problem (DSP). They develop a homotopy method for this. This is then implemented in a bisection search algorithm for solving a robust Bellman update, where each iteration solves the DSP at the midpoint.
    \item \cite{ho2021partial}: $(s, a)$- and $s$-rectangular ambiguity sets defined by the weighted $L_1$ norm, i.e.\ $\|\bm{x}\|_{1, \bm{w}} = \sum_{i=1}^n w_i |x_i|$. Algorithm - partial policy iteration. Policy improvement consists of solving the robust Bellman update, and then choosing a greedy policy which has worst-case value functions equal to to the values just obtained. Then the greedy policy is evaluated in the next step, to get the next value estimates. This is done by optimising the values for the fixed policy. It separates finding the values and finding the policies. Algorithm approximates policy evaluation, where typical policy iteration does it exactly. For $(s, a)$-rectangular sets, the Bellman operator is computed via a homotopy algorithm. For $s$-rectangular sets, it is computed via a bisection search algorithm. Very similar idea to \cite{Ho21} and \cite{ho2022robust}.    
    \item \cite{Grand_Clement_Kroer_2021}: first order methods paper that~\cite{ho2022robust} compared their methods with. First order method algorithm based on similar methods for solving static two-player zero-sum games. Focuses on ellipsoidal ($\ell_2$ norm) and KLD ambiguity sets. The idea of their algorithm is that solving the RMDP boils down to solving $S$ bilinear saddle point problems. 
    \item \cite{ho2022robust}: the paper this one is inspired by. Considers $s$-rectangular ambiguity sets defined by $\phi$-divergences. Focuses of value iteration as opposed to policy iteration as was the case for the last 2. Robust Bellman updates are solved via bisection, where the bounds are updated via solving simplex projection problems. The projection problems are dualised and converted into either univariate convex optimisation problems or bivariate problems where one variable has only a small number of potential values given the other one. Primal dual first order methods are used for solving these problems.
\end{enumerate}
Robust value iteration in particular:
\begin{enumerate}
    \item Already cited, but \cite{GIVAN2000}, \cite{Iyengar05}, \cite{Nilim05} first papers on efficient RVI, all distance based  finite scenarios, interval matrix bounds, ellipsoids, the relative entropy, the KL divergence and maximum a posteriori models.
    \item Already cited, but \cite{xiao2013robust}: interval matrix bounds as well as likelihood uncertainty models.
    \item Already cited, \cite{Zhang2015RobustMD}.
    \item Already cited, but \cite{ho2022robust}, \cite{Grand_Clement_Kroer_2021} etc.
    \item \cite{PetrikRL}: studies the use of robustness for solving aggregated MDPs in reinforcement learning. Commonly in RL, when the state space is large, states are aggregated. This can lead to a reduction in solution quality, since the resulting value function is only approximate. After aggregating the state space, the authors solve a RMDP on the new state space instead of an MDP. The ambiguity set is defined using the $L_1$. They derive performance-loss guarantees and show that robustness improves the amount of loss compared with solving a regular MDP. 
\end{enumerate}
Applications:
\begin{enumerate}
    \item \cite{PaatAssort12}: an assortment optimisation problem, i.e.\ modelling a business deciding which assortment of products to offer customers in order to maximise revenue. Customer choices upon arrival into the system are governed by the multinomial logit choice model, with unknown parameters. MDP model used is a capacity allocation problem - a fixed capacity must be allocated to each of the product categories over a finite horizon in order to try to match customer preferences. Ellipsoidal uncertainty sets for the parameters of the logit choice model. Maybe this is actually quite similar to PDRO, although the parameters are simply customer weights and I am not sure they particularly affect the distribution. Not many details on algorithms given.
    \item \cite{xiao2013robust}: already discussed.
    \item \cite{Zhang2015RobustMD}: RMDP model for medical treatment decision making. State is the health state of the patient, action is which treatment to start them on at that time point. Uncertainty is induced due to not knowing the effect of the treatment, and robustness is required because the effect varies from patient to patient. Finite horizon model with ambiguity sets defined by intervals for the probabilities and uncertainty budgets. Since it is a finite horizon model, it is solved using the RDP algorithm of~\cite{Iyengar05}.
    \item \cite{HuangWindPower}: RMDP model for scheduling the charging of electronic vehicles in a network of charging stations powered by wind power generators. Problem formulated as a robust shortest path problem. Motivation for using robust approach is that the actual amount generated by the windmills is unknown, and it forecasting error can lead to insufficient power for charging the vehicles that require charging. Solved using robust simulation-based policy improvement. Ambiguity set limits the prediction error of the models. Seems as though the uncertainty set does not contain distributions but more point values for the prediction of wind power supply. 
    \item \cite{Goh18Medical}: application of RMDPs to assessing the cost-effectiveness of medical innovations. They discuss element-wise interval uncertainty, weighted distance from nomial distribution (absolute difference, not $\phi$-divergence), weighted combinations of multiple data-based estimates, and sets enforcing element-wise correlation between rows.
    \item \cite{GC_hospitals}: modelling the evolution of patient healthcare in order to proactively decide when patients should be transferred to ICU. Motivation for robustness is that failing to send them in time can lead to greater mortality rates, sending them early is not so damaging. Not rectangular ambiguity sets - the ambiguity sets for different states are correlated and dependent upon a factor model. Ambiguity sets are therefore the factor matrix ambiguity sets of~\cite{goyal2022robust}.
    \item \cite{XinInventory}: RMDP model for inventory control when demand evolves as a martingale. This means the expected demand for today is equal to yesterday's demand. Solved via robust DP, and closed form solutions are actually derived in this case. The ambiguity sets do not seem to be at all constrained in terms of distance, but of course the mean is fixed. This means the ambiguity set changes every day.
\end{enumerate}
DRMDPs:
\begin{enumerate}
    \item \cite{XuDRMDP}: an initial DRMDP paper with ambiguity sets that have a nested structure, enforcing increasingly strong probabilistic guarantees as the sequence progresses. They show that solving the DRMDP can be reduced to solving a RMDP with a single ambiguity set.
    \item \cite{ChenDR}: DRMDPs with rectangular ambiguity sets. They study moment based and distance based ambiguity sets, along with mixture distribution ambiguity sets. Results and reformulations given for both finite and infinite horizon cases. Solution is obtained via solving a collection of robust optimisaition problems in backward DP fashion.
    \item \cite{clementFOM}: The authors of~\cite{Grand_Clement_Kroer_2021} build on their method by extending it to the case of DRMDPs with Wasserstein ambiguity sets. Very similar to their original algorithm.
\end{enumerate}
We can also add some DRO and newsvendor references in a final paragraph, highlighting that our work is connected to those areas. Not sure they need their own section here as this is an RMDP paper with a NV problem as an example. It is not an NV paper or a DRO paper.

==> finite.tex <==
\section{Finite Horizon Model}

In a finite horizon model, we consider $t \in \m{T} = \{0,1,\dots,T\}$. Now, to capture the potential time dependence of the rewards $r$, we write $r^t_{s, a, s'}$ to denote the one-period reward from selecting action $a$ in state $s$ and moving to state $s'$. Furthermore, we now assume that the action space for epoch $t$ is dependent on $S^t$. We now have a sequence $\{\m{A}(s)\}_{s\in \m{S}}$ of action spaces.  In addition, at epoch $t$ we aim to find the policy $\bm{\pi}^t = (\bm{\pi}_s^t)_{s\in \m{S}}$. In other words, $\bm{\pi}^t$ is a vector of policies $\bm{\pi}_s^t = (\pi^t_{s, a})_{a \in \m{A}(s)} \in \Delta_{|\m{A}(s)|}$ for each $s \in \m{S}$ such that $\pi^t_{s, a}$ is the probability that we take action $a \in \m{A}(s)$ when in state $s \in \m{S}$ at time $t \in \m{T}$. A full policy for the problem is given by $\bm{\pi} = (\bm{\pi}_1,\dots, \bm{\pi}^T)$. The set of admissible policies is:
\begin{equation}
    \Pi \subseteq \l( \Delta_{|\m{A}(1)|)} \times \dots \times \Delta_{|\m{A}(S)|}\r)^{T + 1}
\end{equation}
Furthermore, define $\bm{P}_s^t = (P^t_{s, a, s'})_{a \in \m{A}(s), s' \in \m{S}} \in \m{P}_s$ as a transition matrix such that $P^t_{s, a, s'} = \P(S^{t+1} = s'| S^t = s, a^t = a)$ for $a \in \m{A}(s)$, $s' \in \m{S}$ and $t \in \m{T}$. Note that, while the ambiguity set is the same for all epochs, the worst-case distribution for state $s$ is allowed to vary depending on the time point at which we reach the state.

Then, the finite horizon robust model is given by:
\begin{equation}\label{eq:finite_horizon}
    \max_{\bm{\pi} \in \Pi}\min_{\bm{P} \in \m{P}} \E_{\bm{P}, \bm{\pi}}\l[\sum_{t=0}^T \gamma^t r^t_{s^t, a^t, s^{t+1}} \bigg| S^0 \sim \bm{P}^0 \r],
\end{equation}
where $\{(s^t, a^t)\}_{t=0}^T$ is the stochastic process induced by $\bm{\pi}$ and $\bm{P}$ on the space $(\m{S} \times \m{A}^0) \times \dots \times (\m{S} \times \m{A}^T)$ of sample paths. Now let $V^t(s)$ be the value of following an optimal policy from starting in state $s$ at time $t$. Then, the state-wise robust Bellman equations are given by:
\begin{equation}\label{eq:robust_bell_finite}
    V^{t}(s) = \max_{\bm{\pi}_s^t \in \Delta_{|A(s)|}}\min_{\bm{P}_s^t \in \m{P}_s} \sum_{a \in \m{A}(s)} \pi^t_{s, a} \sum_{s' \in \m{S}} P^t_{s, a, s'} \l(r^t_{s, a, s'} + \gamma V^{t+1}(s')\r) \fa s \in \m{S}. 
\end{equation}
We can therefore solve the robust MDP using backward DP as follows:
\begin{enumerate}
    \item Initialise terminal value $V^T(s) \fa s \in \m{S}$, set $t=T-1$.
    \item Calculate the LHS of~\eqref{eq:robust_bell_finite} for each $s \in \m{S}$.
    \item If $t > 0$ then set $t=t-1$ and go to step 2. Else stop.
\end{enumerate}

==> images_tables/pois_actions.tex <==
\begin{tabular}{rrrr}
\toprule
 $s$ &    PBS &    NBS &  100(PBS - NBS) / NBS \\
\midrule
   0 &  2.407 &  2.148 &                12.073 \\
   1 &  1.663 &  1.449 &                14.748 \\
   2 &  1.614 &  1.378 &                17.084 \\
   3 &  1.583 &  1.340 &                18.098 \\
   4 &  1.610 &  1.287 &                25.042 \\
   5 &  1.366 &  1.170 &                16.786 \\
   6 &  1.583 &  1.386 &                14.251 \\
   7 &  1.783 &  1.707 &                 4.456 \\
   8 &  1.598 &  1.813 &               -11.868 \\
   9 &  1.887 &  2.045 &                -7.771 \\
  10 &  1.363 &  1.567 &               -12.983 \\
  11 &  1.961 &  1.623 &                20.809 \\
  12 &  2.574 &  2.421 &                 6.298 \\
  13 &  2.282 &  3.141 &               -27.347 \\
  14 &  2.384 &  3.518 &               -32.239 \\
\bottomrule
\end{tabular}

